On the abandonment and survival of open source projects: An empirical investigation

Background: Evolution of open source projects frequently depends on a small number of core developers. The loss of such core developers might be detrimental for projects and even threaten their entire continuation. However, it is possible that new core developers assume the project maintenance and allow the project to survive. Aims: The objective of this paper is to provide empirical evidence on: 1) the frequency of project abandonment and survival, 2) the differences between abandoned and surviving projects, and 3) the motivation and difficulties faced when assuming an abandoned project. Method: We adopt a mixed-methods approach to investigate project abandonment and survival. We carefully select 1,932 popular GitHub projects and recover the abandoned and surviving projects, and conduct a survey with developers that have been instrumental in the survival of the projects. Results: We found that 315 projects (16%) were abandoned and 128 of these projects (41%) survived because of new core developers who assumed the project development. The survey indicates that (i) in most cases the new maintainers were aware of the project abandonment risks when they started to contribute; (ii) their own usage of the systems is the main motivation to contribute to such projects; (iii) human and social factors played a key role when making these contributions; and (iv) lack of time and the difficulty to obtain push access to the repositories are the main barriers faced by them. Conclusions: Project abandonment is a reality even in large open source projects and our work enables a better understanding of such risks, as well as highlights ways in avoiding them.

==> ecosystems.tex <==
\section{Origin of new TF developers}
\eleni{For now, I keep this section isolated - no reference in any other place until it is finalized - the only reference is in the paper.tex to include the file in the manuscript}
The interview results highlighted the importance of new TF developers who take over the maintenance of projects abandoned by their TF developers. Since our survey results reflect the views of the 33 respondents, we also conducted a quantitative analysis to recover the origin of new TF developers. This analysis is based on the collection of projects of the RubyGems ecosystem, i.e., the package manager of the Ruby programming language. RubyGems was selected for the following reasons: 1) a previous study has shown that RubyGems has faced problems retaining its contributors over the past few years~\cite{Constantinou2017} and 2) as the projects are connected via dependencies between them, we can trace new TF developers who were using the project via such dependencies.

To this end, we used two datasets to perform this analysis in the RubyGems ecosystem. Firstly, we used the Libraries.io dataset\footnote{\url{https://doi.org/10.5281/zenodo.1196312}} to acquire both the GitHub repositories of packages, as well as the dependency information for each package. Next, we repeated all our analysis steps to clone and analyze the projects the GitHub repositories, filter projects based on their commit longevity or deletion from GitHub and perform the TF calculations, as listed in Section~\ref{sec:TF}. The initial dataset consists of 86,245 repositories for 92,472 packages, while after the filtering step we analyze 21,393 GitHub repositories. 

